Pic2Word: Mapping Pictures to Words for Zero-shot Composed Image Retrieval

In Composed Image Retrieval (CIR), a user combines a query image with text to describe their intended target. Existing methods rely on supervised learning of CIR models using labeled triplets consisting of the query image, text specification, and the target image. Labeling such triplets is expensive and hinders broad applicability of CIR. In this work, we propose to study an important task, Zero-Shot Composed Image Retrieval (ZS-CIR), whose goal is to build a CIR model without requiring labeled triplets for training. To this end, we propose a novel method, called Pic2Word, that requires only weakly labeled image-caption pairs and unlabeled image datasets to train. Unlike existing supervised CIR models, our model trained on weakly labeled or unlabeled datasets shows strong generalization across diverse ZS-CIR tasks, e.g., attribute editing, object composition, and domain conversion. Our approach outperforms several supervised CIR methods on the common CIR benchmark, CIRR and Fashion-IQ. Code will be made publicly available at https://github.com/google-research/composed_image_retrieval.

==> paragraphs/exp_keep.tex <==

\input{tables/coco}
\section{Experiments}
\vspace{-2mm}
In this section, we describe experiments evaluating \ours on zero-shot composed image retrieval. We leverage four datasets to assess the performance of the model in diverse scenarios, including the standard CIR benchmarks CIRR~\cite{liu2021image} and Fashion-IQ~\cite{wu2021fashion}.
This section is organized as follows: (i) an explanation of the experimental setup, (ii) an introduction of the main results, and (iii) a detailed analysis. 

\input{figures/ex_coco}
\subsection{Setup}
\textbf{Training Details.}
Unless otherwise stated, we use ViT-L/14 CLIP~\cite{radford2021learning} model pre-trained with LAION-400M~\cite{schuhmann2021laion}.\footnote{We employ \href{https://openaipublic.azureedge.net/clip/models/b8cca3fd41ae0c99ba7e8951adf17d267cdb84cd88be6f7c2e0eca1737a03836/ViT-L-14.pt.}{ViT-L/14} published by OpenAI.}
We train the mapping network on the Conceptual Caption dataset~\cite{sharma2018conceptual}, consisting of 3M images. 
The mapping network consists of three-layered MLP of 512 hidden units with ReLU activation (no activation on the output units). We use AdamW~\cite{loshchilov2018decoupled} with $10^{-4}$ learning rate and $0.1$ weight decay. The batch size of the contrastive learning is 1024. The mapping network is trained on 8 Tesla V100 GPUs. We report the performance averaged over three trials.

\noindent\textbf{(a). Domain conversion.}
In this setup, we evaluate the ability to compose domain information and query image representation. %The task is to retrieve images which are consistent with the content and domain specified by the query image and text respectively.
We utilize ImageNet~\cite{deng2009imagenet} and ImageNet-R~\cite{hendrycks2021many}, which is comprised of 200 classes with diverse domains and has domain annotations. Considering the noise in the annotation, we pick \textit{cartoon, origami, toy and sculpture} as the evaluation target. Then, given the real image from ImageNet and target domain name, we compose the query following the procedure in (a) in Sec~\ref{sec:compose}. %e.g., \texttt{a cartoon of [*]}, where \texttt{[*]} is replaced with a pseudo language token. 
We regard the retrieved image as correct if its class and domain match with the query image and domain. Due to the lack of datasets that can evaluate instance-level cross-domain retrieval on diverse samples, we rely on  class- and domain-level evaluation. While not ideal this evaluation can still give us good insights into the model's ability to accurately translate the domain of the query image compared to baselines.  
The search is performed on 16,983 images from ImageNet-R and ImageNet, i.e., \textit{cartoon, origami, toy, sculpture and real} images are candidates. 

\input{tables/cirr_test}
\input{figures/ex_cirr}

%considering realistic scenario where we have to retrieve target images from the pool of diverse images. 

\noindent\textbf{(b). Object composition.}
We evaluate the ability to compose an instance, given as an image, and other scenes or objects, described by text.
Following Neculai~\etal~\cite{neculai2022probabilistic}, who use COCO~\cite{lin2014microsoft} for composed image retrieval, COCO validation set (5,000 images) is used for evaluation. To create a query for each image, we randomly crop one object and mask its background using its instance mask. The list of object classes, including the class of the query image, in the image is used as text specification. Given the reference image and class list, we compose query by following (b) in Sec~\ref{sec:compose}, e.g., \texttt{a photo of [*], [car], [cat], and dog}.

\noindent\textbf{(c). Scene manipulation by text description.}
CIRR~\cite{liu2021image} (Fig.~\ref{fig:ex_cirr}) is employed to evaluate image manipulation described by text. The modification from the reference to the target image is given as a sentence. We follow the standard evaluation protocol and compose query text following (c) in Sec~\ref{sec:compose}. We report the results on the test split only in Table~\ref{tab:cirr_test}, the validation split is used in other analysis.



\noindent\textbf{(d). Fashion attribute manipulation.}
Fashion-IQ~\cite{wu2021fashion} is employed to evaluate the manipulation of fashion images. The attribute manipulation is given as a sentence.
Similarly to CIRR, we follow the standard evaluation protocol and compose query text following (c) in Sec~\ref{sec:compose}. The validation set is used for evaluation following previous work~\cite{baldrati2022effective}.

\textbf{Zero-shot baselines.}
We provide three zero-shot baselines to fairly compare with our approach. 
\begin{itemize}
    \item \textbf{Image Only.} This baseline retrieves images by computing similarity between target image features and  query image features. 
    \vspace{-2mm}
    \item \textbf{Text Only.} This baseline employs text features only to compute similarity with target images. 
    \vspace{-2mm}
    \item \textbf{Image and Text Baseline.} This baseline utilizes the mean of image and text features as query features. Before taking the average, both image and text features are normalized to have a unit $L_2$-norm.
\end{itemize}

\textbf{Supervised baselines.} To better understand the performance of zero-shot methods, we compare with baselines trained with labeled triplets of a CIR dataset. We implement Combiner~\cite{baldrati2022effective} model with a CLIP ViT-L/14 backbone following the author's code.\footnote{\url{https://github.com/ABaldrati/CLIP4CirDemo}} We train the model with the training split of CIRR or Fashion-IQ; approximately, CIRR has 28,000 training triplets and Fashion-IQ includes 18,000. We also show the reported performance of several CIR methods for CIRR and Fashion-IQ. 

\input{tables/fashion_iq}
\input{figures/ex_fashion}
\input{figures/plots_analysis}


%\input{tables/dataset_comparison}

\input{figures/more_examples}
\input{figures/failure_cases}

\subsection{Main Results}
Tables~\ref{tab:imgnet}-\ref{tab:fashion} present quantitative results, Fig.~\ref{fig:ex_imgnet}-\ref{fig:ex_fashion} illustrate qualitative results. In the experiment on domain conversion using ImageNet (Table~\ref{tab:imgnet}), \ours outperforms all of the baselines with a large margin. This indicates the superiority of \ours in composing domain words and image features. Fig.~\ref{fig:ex_imgnet} demonstrates that \ours captures both the domain and image representations well. 

In the experiment on object composition using COCO (Table~\ref{tab:coco}), \ours outperforms the zero-shot baselines.  Combiner~\cite{baldrati2022effective} trained on Fashion-IQ performs better than \ours while the model trained on CIRR performs worse than \ours. A model trained on one dataset is not necessarily transferable to other datasets because each composed retrieval dataset can require different dataset bias, e.g., relative importance of image features and caption features. 

On scene and fashion attribute manipulation datasets, e.g., CIRR and Fashion-IQ, \ours outperforms zero-shot baselines and some of the supervised approaches. 
For these datasets, we observe that the captions alone can be informative enough to retrieve the correct target images (e.g., last row in Fig.~\ref{fig:ex_cirr}), and that some reference images are not very relevant to the target image. 
Then, the supervised model can learn the dataset-specific bias on how to combine the two modalities. For example, the model can prioritize learning from text or ignoring the reference image if the image and text are not related well.
We hypothesize that this is affecting the transferability of the supervised models. 
More detailed analysis is provided in the following section.
%Zero-shot models cannot learn such a dataset bias. 

\subsection{Analysis}
\label{sec:analysis}
\textbf{Does the pseudo language token capture the image information?}
To analyze the information in the estimated token, we conduct evaluation using CC3M validation 13,164 images. Concretely, we evaluate whether the language embedding generated by the pseudo token can retrieve the input image. Recall at top 1 and 5 is 99.8 and 100.0 respectively, indicating that the token captures the unique image features very well. 

\textbf{Insights on existing composed retrieval datasets.}
The results on CIRR and Fashion-IQ (Table~\ref{tab:cirr_test} and ~\ref{tab:fashion}) imply that some target images can be correctly retrieved just by using text. We find that reference images can be irrelevant to text query or text query is informative enough to search target image. This relative importance of reference image and text is a dataset-specific bias. We investigate the importance in Fig.~\ref{fig:weight_study}, where we produce a query embedding by varying the interpolation weight, $w$, in computing the average of text $t$ and image features $v$, i.e., $q = w * t + (1-w) * v$. The result indicates that the optimal weight can be unique to each dataset and the performance is sensitive to the weight parameter. A supervised method can learn the relative importance from labeled triplets, but it is hard to learn for a zero-shot method. 

\textbf{Comparison to supervised baseline with fewer training samples.}
Fig.~\ref{fig:fashion_num_sample} and \ref{fig:cirr_num_samples} show the performance of the supervised baseline (Combiner~\cite{baldrati2022effective}) with fewer training samples. Overall, our approach outperforms the baseline if fewer than 1,000 triplets are given as training samples.



\textbf{More qualitative examples.}
Fig.~\ref{fig:interesting} shows retrieval results using CC3M validation data. 
Our model can compose images with adjective (second) or a place (third) and read the style given as an image (bottom). 

\textbf{Failure cases.}
One of the popular applications is sketch-based image retrieval~\cite{liu2017deep}, where the user draws a sketch to retrieve natural images, as shown in Fig.~\ref{fig:failures}.
Qualitatively, retrieving an image from a non-natural image domain is likely to be successful (bottom two) while retrieving natural images from sketch images is not trivial (top two). 
Prompts other than \texttt{a real image of} do not work well for this task either. Natural images are not described with a domain word in pre-training image-caption dataset while other domains, e.g., art, cartoon, sketch and origami, are often described with corresponding domain name. An appropriate domain description for natural images may not exist. 

==> tables/cirr.tex <==
\begin{table}[t]
  \centering 
  \scalebox{0.9}{
  \begin{tabular}{c|c|cccc} 
  \toprule
  \cmidrule{1-5}
  \multicolumn{1}{l}{Supervision} & \multicolumn{1}{c}{Methods} & R1& R5&R10&R50\\ 
  \midrule
  %\multirow{8}{*}{\rotatebox{90}{\textsc{Baselines}}}
   \multirow{4}{*}{{\textsc{Zero-shot}}} & Image-only    &7.5&25.1&	35.5&59.8\\ 
   & Text-only   &20.8&46.2&57.0&78.8\\
   & Image$+$Text  &13.2&36.6&50.5&78.1\\
   & \ours &\textbf{22.6}&\textbf{52.6}&\textbf{66.6}&\textbf{87.3}\\
     \cmidrule{1-6}
  \multicolumn{1}{c|}{CIRR} &Combiner&33.1&65.8&77.8&94.0\\
  \multicolumn{1}{c|}{Fashion-IQ}&Combiner&16.9&44.4&58.5&85.2\\
%  \multicolumn{1}{c|}{CIRR}&CIRPLANT~\cite{liu2021image}&19.6&52.6&68.4&92.4\\
   \multicolumn{1}{c|}{CIRR}&ARTEMIS&N/A&49.0&N/A&89.2\\
  \bottomrule
  \end{tabular}}
  \caption{Evaluation on CIRR validation set.}
  \label{tab:cirr}
\end{table}






==> tables/dataset_comparison.tex <==
\begin{table}[t]
  \centering 
  \scalebox{0.7}{
  \begin{tabular}{c|cccc} 
  \toprule
  \cmidrule{1-5}
  \multirow{2}{*}{Training Dataset} &  ImageNet & COCO &CIRR& Fashion      \\ 
  &R100&R1&R1&R10\\
  \midrule
  %\multirow{8}{*}{\rotatebox{90}{\textsc{Baselines}}}
  CC3M    &\textbf{31.1}&\textbf{11.7}&22.6&\textbf{26.3}\\ 
  CC12M & 29.1&11.3&\textbf{23.5}&25.8\\
  ImageNet21K&19.6&9.4&20.6&25.5\\
  \bottomrule
  \end{tabular}}
  \caption{\textbf{Study on the dataset used to train mapping network.}}
  \label{tab:dataset}
\end{table}


==> tables/table_template.tex <==
\begin{table*}[!ht]
  \centering \scalebox{0.8}{
  \begin{tabular}{lllrrrr} 
  \toprule
  \multicolumn{2}{c}{} & \multicolumn{1}{c}{}        & \multicolumn{4}{c}{Recall$@K$ } \\
  \cmidrule(lr){4-7}
  \multicolumn{2}{l}{} & \multicolumn{1}{l}{Methods} & $K=1$           & $K=5$           & $K=10$ & $K=50$     \\ 
  \midrule
  %\multirow{8}{*}{\rotatebox{90}{\textsc{Baselines}}}
  & 1 & Image-only                   \\
  & 2 & Text-only                   \\
  & 3 & Image$+$Text                  \\
  \cmidrule{2-7}
  & 4 & \ours                  \\
  \bottomrule
  \end{tabular}}
  \caption{}
  \label{tab:baseline_0}
\end{table*}
